Barless flocculent galaxies: a dynamic puzzle

We draw attention to the bright galaxies that do not show a bar in their structure but have a flocculent spiral structure. Using the THINGS' and HERACLES' kinematic data for four barless galaxies (NGC~2841, NGC~3512, NGC~5055, NGC~7331) we built their mass models including dark halos. We concluded that the fraction of the dark matter does not exceed 50\% within the optical radii of the galaxies. This is too little to explain the lack of a bar in these galaxies. In an attempt to understand the featureless structure of these galaxies we constructed several $N$-body models with an initially reduced content of dark matter. We concluded that, in addition to the low mass of the dark halo, the decisive factor that leads to a barless disc is the start from an initially unstable state. An isolated dynamically cold disc (with the Toomre parameter $Q < 0.5$) settled into rotational equilibrium passes trough the short stage of violent instability with fragmentation and formation of stellar clumps. After that, it evolves passively and ends up with a featureless structure. We assume that the barless flocculent galaxies studied in the present work may be descendants of galaxies at high redshifts with rotation curves which are consistent with the high mass fraction of baryons relative to the total dark matter halo.

==> latexmkrc <==
$ENV{'TEXINPUTS'}='./sty//:' . $ENV{'TEXINPUTS'}; 

# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

==> pgfgraphicsmacros.tex <==
\usepackage{adjustbox} 
\usepackage{import} 
% i know what i'm doing!
\makeatletter
\def\import@pgf@picture#1\@end{%
  \def\@dir{}\def\@file{}%
  \parse@paths#1/\relax/%
  \expandafter\expandafter\expandafter\import%
  \expandafter\expandafter\expandafter{\expandafter\@dir\expandafter}\expandafter{\@file}%
} % adapted parser by David Carlisle, https://tex.stackexchange.com/a/84804
\def\parse@paths#1/#2/{%
  \edef\@trailing{#2/}%
  \ifx\relax#2\edef\@file{#1}\edef\@trailing{}%
  \else \edef\@dir{\@dir#1/}\expandafter\expandafter\expandafter\parse@paths\expandafter\fi\@trailing%
}
% \def\@import@pgf@picture#1/#2\@end{\import{#1}{#2}}
\newcommand*{\includepgfgraphics}[2][]{%
  \begingroup%
  \ifx &#1&\import@pgf@picture #2\@end%
  \else \begin{adjustbox}{#1}\import@pgf@picture #2\@end\end{adjustbox}%
  \fi\endgroup%
}
\makeatother

==> reviewmacros.tex <==
% setup authorship colors
\RequirePackage{xcolor}
\RequirePackage{etoolbox}

\makeatletter
\newwrite\@todofile
\AtBeginDocument{\immediate\openout\@todofile=todo.txt}
\AtEndDocument{\immediate\closeout\@todofile}
\newcommand*{\todo}[3][]{%
  \begingroup%
  \edef\@isdone{#1}\def\@donestring{done}\def\@doneflag{}%
  \edef\@authors{#2}\def\@task{#3}%<-- not expand this one
  \def\do##1{@##1\space}%
  \def\printauthors{%
    \expandafter\docsvlist\expandafter{\@authors}%
  }%
  \ifdefstrequal{\@isdone}{\@donestring}{%
    \def \@doneflag{x\space}%
    [\textcolor{lightgray}{\texttt{\printauthors \textbf{:} \@task}}]%
  } {[\texttt{\textcolor{red}{\textbf{\printauthors}}\textbf{:} \@task}]}%
  \immediate\write\@todofile{\@doneflag \expandonce{\@task} \space \printauthors}%
  \endgroup%
}
\makeatother

\newcommand*\asc[1]{[{\textcolor{blue}{AS suggests: {#1}}}]}
\newcommand*\ascsc[1]{[{\textcolor{blue}{AS: {#1}}}]}
\let \ascs = \ascsc
%\newcommand*\asen[1]{[{\textcolor{green}{Eng problem: {#1}}}]}
\newcommand*\ascwc[2]{[\textcolor{blue}{#1} {\textcolor{blue}{Suggest: {#2}}}]}
\newcommand*\asen[1]{\textcolor{red}{#1}}
%\newcommand*\asw[1]{[{\textcolor{blue}{AS suggests: {#1}}}]}

% colors
\newcommand{\setnamecolor}[2]{
  \def\do##1{\colorlet{reviewcolors@##1}{#2}}
  \docsvlist{#1}
}
\definecolor{fuchsia}{rgb}{1.0, 0.0, 1.0}
\setnamecolor{Ilia,Iliya,Ilya,IT}{fuchsia!50!black}
%\setnamecolor{Anton,AS}{blue}
\setnamecolor{Reviewer}{magenta}
\setnamecolor{Authors}{red}
\setnamecolor{SS}{fuchsia!50!black}
\setnamecolor{Daria}{red!50!black}
\setnamecolor{NS,NYa}{green!50!black}
\setnamecolor{Anton}{black}

% #1 = text that is commented
% #1 = author
% #2 = body of comment.
% You may use \c1 \c2 \c3 etc anchors both in the commented text and in the body of the comment.
\newcommand*{\reducedstrut}{\vrule width 0pt height .9\ht\strutbox depth .9\dp\strutbox\relax}
\newcommand*{\commenttextpieces}[3]{%
  \begingroup%
  \setlength{\fboxsep}{0pt}% 
  \def\c##1##2{%
    \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
    \colorbox{reviewcolors@#2!15}{%
      \reducedstrut%
      \mathifmathoutside{##2}%
      \/%italic correction
      \hbox to 0pt{${}^{\textcolor{reviewcolors@#2}{##1}}$}%
    }}%
  #1%
  \def\c##1{\hbox{${}^{\text{##1}}$}}%
  \thinspace[\textcolor{reviewcolors@#2}{(\textbf{#2}) #3}]%
  \endgroup%
}

\makeatletter
\newcommand*{\startcommenting}[1][]{
  \begingroup
  \let \summary=\commenting@create@summary
  \let \nosummary=\commenting@omit@summary
  \ifblank{#1}%
    {\def\@commenting@author{anon}}
    {\def\@commenting@author{#1}}
  \setlength{\fboxsep}{0pt}% 
  \let \c=\commenting@make@comment
  \let \ins=\commenting@suggest@insert
}
\newcommand*{\commenting@make@comment}[2]{%
  \ifmmode \let \mathifmathoutside=\ensuremath \else \let\mathifmathoutside=\relax \fi%
  \colorbox{reviewcolors@\@commenting@author!15}{%
    \reducedstrut%
    \mathifmathoutside{#2}%
    \/%italic correction
    \hbox to 0pt{${}^{\textcolor{reviewcolors@\@commenting@author}{#1}}$}%
  }}%
\newcommand*{\commenting@suggest@insert}[1]{%
  \textcolor{reviewcolors@\@commenting@author}{#1}%
}
\newcommand{\commenting@annotate@label}[1]{%
  \hbox{${}^{\text{#1}}$}%
}
\newcommand*{\commenting@create@summary}[2][\@commenting@author]{%
  \let \c=\commenting@annotate@label
  \let \ins=\relax
  \thinspace[\textcolor{reviewcolors@#1}{(\textbf{#1}) #2}]%
  \endgroup%
}
\newcommand*{\commenting@omit@summary}{%
  \endgroup%
}
\makeatother

\newcommand*\note[2]{[{\color{reviewcolors@#1}(\textbf{#1})\  #2}]}
